Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems

Industry 4.0 offers many possibilities for creating highly efficient and flexible manufacturing. To create such advantages, highly automated and thus digitized processes and systems are required. Here, most technologies known from the office floor are basically suitable for these tasks, but cannot meet the high demands of industrial use cases. Therefore, they cannot replace industrial technologies and devices that have performed well over decades "out of the box". For this reason, many technologies known from the office floor are being investigated and adapted for industrial environments. An important task is the virtualization of process controls, as more and more devices use computation offloading, e.g. due to limited resources. In this paper we extend the work on our novel architecture that enables numerous use cases and meets industrial requirements by virtualizing process controllers. In addition, a testbed based on a factory scenario is proposed to evaluate the most important features of the presented architecture.

==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/IEEE_authors-long.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Michael Gundall\IEEEauthorrefmark{1}, %
   % Daniel Reti\IEEEauthorrefmark{1}, %
    Calvin Glas\IEEEauthorrefmark{1}, %
    and Hans D. Schotten\IEEEauthorrefmark{1}\IEEEauthorrefmark{2} %
    \\%
  %  FirstName1 Lastname1\IEEEauthorrefmark{3} and %
   % FirstName2 Lastname2\IEEEauthorrefmark{4}%
}%
\IEEEauthorblockA{%
    \IEEEauthorrefmark{1}German Research Center for Artificial Intelligence GmbH (DFKI), \\ Kaiserslautern, Germany \\% 
  %  \IEEEauthorrefmark{2} Department of Computer Science, Technische Universität Kaiserslautern, \\ Kaiserslautern, Germany \\%
    \IEEEauthorrefmark{2}Department of Electrical and Computer Engineering, Technische Universität Kaiserslautern, \\ Kaiserslautern, Germany %
%     Trippstadter Str. 122\\%
%     67663 Kaiserslautern\\%
	\\%
  %  \IEEEauthorrefmark{3}Institute1, %
  %  Some Subtitle 1 %
%     Optional Address, Germany%
 %   \\%
	%\IEEEauthorrefmark{4}Corporation2, %
  %  Some Subtitle2, %
  %  Some more Subt2 %
%     Optional Address
  %  \\%
    Email: %
        \{michael.gundall, %daniel.reti, 
        calvin.glas, hans\_dieter.schotten%
        \}@dfki.de%, %
        \\%
    %    c\_glas15@informatik.uni-kl.de
     %   \\
      %  \IEEEauthorrefmark{3}Mail1@domain1.de, %
      %  \IEEEauthorrefmark{4}Mail2@domain2.com
}%
}%






% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Michael Gundall\IEEEauthorrefmark{1},\\%
    %Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%








% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/_templates/IEEE_authors-long.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1}, %
    Christoph Fischer\IEEEauthorrefmark{2}, %
    \\%
    FirstName1 Lastname1\IEEEauthorrefmark{3} and %
    FirstName2 Lastname2\IEEEauthorrefmark{4}%
}%
\IEEEauthorblockA{%
    \IEEEauthorrefmark{1}\IEEEauthorrefmark{2}German Research Center for Artificial Intelligence GmbH (DFKI)%
%     Trippstadter Str. 122\\%
%     67663 Kaiserslautern\\%
	\\%
    \IEEEauthorrefmark{3}Institute1, %
    Some Subtitle 1 %
%     Optional Address, Germany%
    \\%
	\IEEEauthorrefmark{4}Corporation2, %
    Some Subtitle2, %
    Some more Subt2 %
%     Optional Address
    \\%
    Email: %
        \{\IEEEauthorrefmark{1}dennis.krummacker, %
        \IEEEauthorrefmark{2}christoph.fischer\}@dfki.de, %
        \\%
        \IEEEauthorrefmark{3}Mail1@domain1.de, %
        \IEEEauthorrefmark{4}Mail2@domain2.com
}%
}%






% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/_templates/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1},\\%
    Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%









%\author{%
%           \IEEEauthorblockN{Michael Shell}
%           \IEEEauthorblockA{School of Electrical and\\Computer Engineering\\
%           Georgia Institute of Technology\\
%           Atlanta, Georgia 30332--0250\\
%           Email: http://www.michaelshell.org/contact.html}
%           \and
%           \IEEEauthorblockN{Homer Simpson}
%           \IEEEauthorblockA{Twentieth Century Fox\\
%           Springfield, USA\\
%           Email: homer@thesimpsons.com}
%           \and
%           \IEEEauthorblockN{James Kirk\\ and Montgomery Scott}
%           \IEEEauthorblockA{Starfleet Academy\\
%           San Francisco, California 96678--2391\\
%           Telephone: (800) 555--1212\\
%           Fax: (888) 555--1212}
%
%}%

% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/backing/IEEETemplateProvidedExamples.tex <==
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
% \begin{table}[!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
% \caption{An Example of a Table}
% \label{table_example}
% \centering
% % Some packages, such as MDW tools, offer better commands for making tables
% % than the plain LaTeX2e tabular which is used here.
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{table}

==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/backing/thebibliography.tex <==
% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
  
\bibitem{IEC61158}
, \emph{IEC 61158},

\bibitem{61158-trafficclass}
E DIN EN 61158-1:2017-09 11.4.2

\bibitem{61158-endpoint}
E DIN EN 61158-1:2017-09 9.3.3.3.1

\bibitem{62439-endnode}
DIN EN 62439-1:2010-09 3.1.13

\end{thebibliography}

==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/makros.tex <==
%
%
%
%
% own command to get a newline, without this disturbing underfull \hbox
% still beware of the "Glue" from the set \parskip height plus x minus y
% which in fact allows latex to stretch the space between paragraphs
% (by default up to 1pt)
\newcommand{\nl}{\par\noindent} % Abk. für NewLine
% and here a command to create really a new paragraph
% inserts an additional free line
\newcommand{\np}{\par\vspace{\baselineskip}} % Abk. für NewParagraph
\newcommand{\npi}{\par\vspace{\baselineskip}\noindent} % Abk. für NewParagraph_noIndent
% Zu benutzen also so:
% Neue Zeile ohne Einrückung: \nl
% Neue Zeile mit Einrückung: Freie Zeile im Editor
% Neuer Absatz mit freier Zeile dazwischen: \na
\newcommand{\greenuline}[1]{\colorlet{temp}{.}\color{green}\underline{\color{temp}#1}\color{temp}\xspace}%
%
%
%
%
%
%
% 
% Makro für Kreis um Text
\newcommand\circlearound[1]{%
  \tikz[baseline]\node[draw,shape=circle,anchor=base,inner sep=0.3ex] {#1} ;}
\newcommand\lipsaround[1]{%
  \tikz[baseline]\node[draw,shape=ellipse,anchor=base,inner sep=0.3ex] {#1} ;}
%
\newcommand\rectdotaround[2]{%
  \tikz[baseline]\node[draw=#1,thick, loosely dotted,%
  shape=rectangle,anchor=base,inner sep=0.5ex] {#2} ;}
%
%
%
%
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%			Verschiedene Definitionen wie Schriftzeichen
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\newcommand{\mytilde}{{\raise.17ex\hbox{$\scriptstyle\mathtt{\sim}$}}}
\newcommand{\mytildeA}{\textasciitilde}
\newcommand{\mytildeB}{$\sim$}
\newcommand{\mytildeC}{\~{}}
\newcommand{\mytildeD}{\texttildelow}
\newcommand{\mytildeE}{\raisebox{-.8ex}{\textasciitilde}}
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							Definitionen fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%

==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/preamble.tex <==
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%							PassOptions Preparation
%	Die PassOptions sollten vor der ersten Inklusion des Packages erfolgen
%	Also auch bevor ein Package von einem anderen eingebunden wird...
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\PassOptionsToPackage{usenames,dvipsnames,svgnames,x11names,table,prologue}{xcolor}%
\PassOptionsToPackage{hyphens}{url}%
\PassOptionsToPackage{nomessages}{fp}%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							PassOptions fertig
%------------------------------------------------------------------------
%========================================================================
%
%
%
%
%
%_____________________________________________________________________________
%=============================================================================
%=============================================================================
%=============== START from IEEE Document-Class Template =====================
%=============================================================================
%-----------------------------------------------------------------------------
%% bare_conf.tex
%% V1.4b
%% 2015/08/26
%% by Michael Shell
%% See:
%% http://www.michaelshell.org/
%% for current contact information.
%%
%% This is a skeleton file demonstrating the use of IEEEtran.cls
%% (requires IEEEtran.cls version 1.8b or later) with an IEEE
%% conference paper.
%%
%% Support sites:
%% http://www.michaelshell.org/tex/ieeetran/
%% http://www.ctan.org/pkg/ieeetran
%% and
%% http://www.ieee.org/

%%*************************************************************************
%% Legal Notice:
%% This code is offered as-is without any warranty either expressed or
%% implied; without even the implied warranty of MERCHANTABILITY or
%% FITNESS FOR A PARTICULAR PURPOSE! 
%% User assumes all risk.
%% In no event shall the IEEE or any contributor to this code be liable for
%% any damages or losses, including, but not limited to, incidental,
%% consequential, or any other damages, resulting from the use or misuse
%% of any information contained here.
%%
%% All comments are the opinions of their respective authors and are not
%% necessarily endorsed by the IEEE.
%%
%% This work is distributed under the LaTeX Project Public License (LPPL)
%% ( http://www.latex-project.org/ ) version 1.3, and may be freely used,
%% distributed and modified. A copy of the LPPL, version 1.3, is included
%% in the base LaTeX documentation of all distributions of LaTeX released
%% 2003/12/01 or later.
%% Retain all contribution notices and credits.
%% ** Modified files should be clearly indicated as such, including  **
%% ** renaming them and changing author support contact information. **
%%*************************************************************************


% *** Authors should verify (and, if needed, correct) their LaTeX system  ***
% *** with the testflow diagnostic prior to trusting their LaTeX platform ***
% *** with production work. The IEEE's font choices and paper sizes can   ***
% *** trigger bugs that do not appear when using other class files.       ***                          ***
% The testflow support page is at:
% http://www.michaelshell.org/tex/testflow/


% \documentclass[conference]{IEEEtran}%
% Some Computer Society conferences also require the compsoc mode option,
% but others use the standard conference format.
%
% If IEEEtran.cls has not been installed into the LaTeX system files,
% manually specify the path to it like:
% \documentclass[conference]{../sty/IEEEtran}

%-------------------------------------------------------------------------------
%-------------------------------------------------------------------------------
%
% \usepackage{etex}%
% \reserveinserts{32}%
%
%-------------------------------------------------------------------------------
%-------------------------------------------------------------------------------



% Some very useful LaTeX packages include:
% (uncomment the ones you want to load)


% *** MISC UTILITY PACKAGES ***
%
%\usepackage{ifpdf}
% Heiko Oberdiek's ifpdf.sty is very useful if you need conditional
% compilation based on whether the output is pdf or dvi.
% usage:
% \ifpdf
%   % pdf code
% \else
%   % dvi code
% \fi
% The latest version of ifpdf.sty can be obtained from:
% http://www.ctan.org/pkg/ifpdf
% Also, note that IEEEtran.cls V1.7 and later provides a builtin
% \ifCLASSINFOpdf conditional that works the same way.
% When switching from latex to pdflatex and vice-versa, the compiler may
% have to be run twice to clear warning/error messages.






% *** CITATION PACKAGES ***
%
%\usepackage{cite}
% cite.sty was written by Donald Arseneau
% V1.6 and later of IEEEtran pre-defines the format of the cite.sty package
% \cite{} output to follow that of the IEEE. Loading the cite package will
% result in citation numbers being automatically sorted and properly
% "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% \cite will automatically add leading space, if needed. Use cite.sty's
% noadjust option (cite.sty V3.8 and later) if you want to turn this off
% such as if a citation ever needs to be enclosed in parenthesis.
% cite.sty is already installed on most LaTeX systems. Be sure and use
% version 5.0 (2009-03-20) and later if using hyperref.sty.
% The latest version can be obtained at:
% http://www.ctan.org/pkg/cite
% The documentation is contained in the cite.sty file itself.






% *** GRAPHICS RELATED PACKAGES ***
%
\ifCLASSINFOpdf
  \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex





% *** MATH PACKAGES ***
%
%\usepackage{amsmath}
% A popular package from the American Mathematical Society that provides
% many useful and powerful commands for dealing with mathematics.
%
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath





% *** SPECIALIZED LIST PACKAGES ***
%
%\usepackage{algorithmic}
% algorithmic.sty was written by Peter Williams and Rogerio Brito.
% This package provides an algorithmic environment fo describing algorithms.
% You can use the algorithmic environment in-text or within a figure
% environment to provide for a floating algorithm. Do NOT use the algorithm
% floating environment provided by algorithm.sty (by the same authors) or
% algorithm2e.sty (by Christophe Fiorio) as the IEEE does not use dedicated
% algorithm float types and packages that provide these will not provide
% correct IEEE style captions. The latest version and documentation of
% algorithmic.sty can be obtained at:
% http://www.ctan.org/pkg/algorithms
% Also of interest may be the (relatively newer and more customizable)
% algorithmicx.sty package by Szasz Janos:
% http://www.ctan.org/pkg/algorithmicx




% *** ALIGNMENT PACKAGES ***
%
%\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array


% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.




% *** SUBFIGURE PACKAGES ***
\ifCLASSOPTIONcompsoc
   \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\else
   \usepackage[caption=false,font=footnotesize]{subfig}
\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig




% *** FLOAT PACKAGES ***
%
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e


\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
%\usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix




% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.
%
%
%
%
%
% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )
%
%_____________________________________________________________________________
%=============================================================================
%=============================================================================
%=============== END from IEEE Document-Class Template =======================
%=============================================================================
%-----------------------------------------------------------------------------
%
%
%
%
%
% Package Includes - maybe some imediate with options
%
%________________________________________________________________________
%------------------------------------------------------------------------
%					Basic Language depending Packages
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\usepackage[english]{babel}%
\selectlanguage{english}%
\usepackage[utf8]{inputenc}%
% \usepackage[T1]{fontenc}%
\usepackage[babel,style=english]{csquotes}%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							END Basic Language
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%							Schriftarten einstellen
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%\usepackage[scaled]{uarial}
% \usepackage{bookman}
%\usepackage{textcomp}%
%------------------------------------------------
%\renewcommand*{\ttdefault}{lmtt}%
%<-------------------->
% Create a command to format as typewrite with enabled hyphenation
% (Silbentrennung)
%<-------------------->
%\makeatletter
%\DeclareRobustCommand\ttfamily
%        {\not@math@alphabet\ttfamily\mathtt
%         \fontfamily\ttdefault\selectfont\hyphenchar\font=-1\relax}
%\makeatother
%\DeclareTextFontCommand{\texttthyph}{\ttfamily\hyphenchar\font=45\relax}
% Standartmäßig verfügbare Schriftarten:
% cmtt 	Computer Modern Typewriter (default)
% lmtt 	Latin Modern
% pcr 	Courier
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							Schriftarten fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%					Some 'Specials', one might want/like
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\usepackage{hyphsubst}%
\usepackage[%
	activate={true,%
	nocompatibility},%
	final,%
	tracking=true,%
	kerning=true,%
	spacing=true,%
	factor=1100,%
	stretch=10,%
	shrink=10%
]{microtype}%
% activate={true,nocompatibility} - activate protrusion and expansion
% final - enable microtype; use "draft" to disable
% tracking=true, kerning=true, spacing=true - activate these techniques
% factor=1100 - add 10% to the protrusion amount (default is 1000)
% stretch=10, shrink=10 - reduce stretchability/shrinkability (default is 20/20)
%\usepackage{todonotes}%
\usepackage{setspace}%
%
%
%
%
% See PassOptions for xcolor on Top
\usepackage{xcolor}%
\definecolor{todonotecol}{RGB}{250,0,0}%
%
%
%
%For \DeclareDocumentCommand (bessere Makro-Definition als \newcommand) and so on
\usepackage{xparse}
%	Also Necessary to create the DualEntry Makro for Glossaries
%
%
%
% See PassOptions for url on Top
\usepackage[%
	colorlinks=false,%
	urlcolor=black,%
	linkcolor=black,%
% 	citecolor=citegreen,%
	citecolor=black,%
	filecolor=black,%
	breaklinks,%
	]{hyperref}%
\usepackage{url}%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							END 'Specials'
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%					Für Abkürzungen, Glossar und weiteres
%						glossaries
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
% Glossaries muss NACH hyperref, babel, polyglossia, inputenc and fontenc geladen werden
% See PassOptions for fp on Top
\usepackage[%
	acronym,%
% 	nomain,%
% 	nonumberlist,%
	nopostdot,%
	seeautonumberlist,%
	shortcuts,%
	section=chapter,%
	toc,%
]{glossaries}%
% \makeglossaries%
\loadglsentries{./supply/glossaries.tex}%
\glsdisablehyper% Disables Hyperlinks
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%					glossaries fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%                   Für Zitate / Quellen:
%                   --- Begin biblatex ---
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\usepackage[%
	backend=biber,%
	style=ieee,%
	isbn=false,%
% 	style=apa,%
% 	apabackref=true,%
	hyperref=true,%
	maxbibnames=99,%
	sorting=none,%
	natbib=true,%
	language=english,%
	defernumbers=true,%
	]{biblatex}%
% \DeclareLanguageMapping{ngerman}{ngerman-apa}%
\DeclareFieldFormat{sentencecase}{\csname bbx@colon@search\endcsname#1}% Therewith capital letters stay capitals, when using 'style=ieee'
\renewcommand*{\bibfont}{\normalfont\footnotesize}
%   One might also want to take a look at 'titlecase', when using 'style=ieee'
\addbibresource{./supply/literature.bib}%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%                   --- End biblatex ---
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%
\usepackage{balance}
%Various (Basic) Packages
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
% \usepackage{subfigure}% Just as Info: subfigure is dead. Use subfig.sty instead, which is loaded above
\usepackage{nameref}
\usepackage{soul}
\usepackage{flushend}
\usepackage{textcomp}
\usepackage{calc}
\usepackage{xkeyval}
\usepackage{multirow}
% \usepackage{ifthen}
%
%%%%\usepackage{tabular}% Latex-Std, just don't use
%\usepackage{tabular*}% Latex-Std, bit better
%%%%\usepackage{tabularx}% More comfortable than, 'tabular*', better to use, but no nesting
\usepackage{tabulary}% Nearly the same as 'tabularx', bit more extensive
\usepackage{makecell}% http://ctan.org/pkg/makecell
%------------------------------------------------------------------------------------
% -- Table recommendation:
% ---- Use 'tabulary', together with 'makecell' (if necessary)
% ---- -- Could also use 'tabularx', together with 'makecell', if you like it better...
% ---- Otherwise maybe 'tabular*'
%------------------------------------------------------------------------------------
%
%------------------------------------------------------------------------------------
% -- Want to use 'tikz' ?  :oD
% - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - - -
\usepackage{pgfplots}
\usepackage{tikz}
\usepackage{textcomp} 
\usepackage{verbatim}

\pgfplotsset{ grid style={
 %   dashed% pattern = on 0.025mm off 0.95mm on 0.025mm off 0mm, % start with half a dot to get correct centering of the pattern
  %  line cap = round,
   % black,
   line width = 0.1pt
  }, compat=1.16}

%------------------------------------------------------------------------------------
%
%\usepackage{marginnote}
%\usepackage{caption}
%\usepackage{subcaption}
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%					
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%					Additional Packages
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\

%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%					
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%

==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/organization/settings.tex <==
%
%
% Setups
%
%
%
%
%		New Lenghts & Variables
\newlength\textheighttemp%
% \setlength{\textheighttemp}{\textheight}%
\newlength\textwidthtemp%
% \setlength{\textwidthtemp}{\textwidth}%
\newlength\textheightstd%
\setlength{\textheightstd}{\textheight}%
\newlength\textwidthstd%
\setlength{\textwidthstd}{\textwidth}%
\newlength\textheightold%
\newlength\textwidthold%
%
\newlength\tempheight%
\newlength\tempwidth%
%
%
%
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%							Setups für Microtype
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\SetProtrusion{encoding={*},family={bch},series={*},size={6,7}}
              {1={ ,750},2={ ,500},3={ ,500},4={ ,500},5={ ,500},
               6={ ,500},7={ ,600},8={ ,500},9={ ,500},0={ ,500}}
\SetExtraKerning[unit=space]
    {encoding={*}, family={bch}, series={*}, size={footnotesize,small,normalsize}}
    {\textendash={400,400}, % en-dash, add more space around it
     "28={ ,150}, % left bracket, add space from right
     "29={150, }, % right bracket, add space from left
     \textquotedblleft={ ,150}, % left quotation mark, space from right
     \textquotedblright={150, }} % right quotation mark, space from left
\SetTracking{encoding={*}, shape=sc}{40}
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							Microtype fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%							Setups für Glossaries
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%Formatierung für Abkürzungen bei erstem Auftreten und weiteren und
%Falls deutsch Key im GLossar vorhanden, benutze ihn beim ersten Mal
% \defglsentryfmt[\acronymtype]{
%   \ifglsused{\glslabel}
%     {\glsgenentryfmt}% Wenn verwendet normales format
%     {\textit{\glsgenentryfmt}}% beim ersten mal kursiv
% }
%       \newcommand*{\glsprintmitdeutsch}{%
%           {\glsentrylong{\glslabel} (\glsentryname{\glslabel}, dt.:
%           \glsentrydeutsch{gls-\glslabel})}%
%       }%
%       \newcommand*{\glsprintmitenglisch}{%
%           {\glsentrylong{\glslabel} (\glsentryname{\glslabel}, engl.:
%           \glsentryenglisch{gls-\glslabel})}%
%       }%
%       \newcommand*{\glsprintmitdualentry}{%
%         \ifglsused{\glslabel}%
%           {%
%               \glsgenentryfmt%
%           }{%
%               \ifglshasfield{deutsch}{gls-\glslabel}{%
%                   \glsprintmitdeutsch%
%               }{%
%                   \ifglshasfield{englisch}{gls-\glslabel}{%
%                       \glsprintmitenglisch%
%                   }{%
%                       {\glsgenentryfmt}%
%                   }%
%               }%
%           }%
%       }%
%       \newcommand*{\glsprintohnedeutsch}{%
%         \ifglsused{\glslabel}%
%           {\glsgenentryfmt}% Wenn verwendet normales format
%           {\glsgenentryfmt}% beim ersten mal anders formatiert
%       }%
%       % Alternativen für erste Formatierung:
%       % textsf, textit, texttt
%       %
%       \defglsentryfmt[\acronymtype]{%
%           \ifglsentryexists{gls-\glslabel}{%
%               \glsprintmitdualentry%
%           }{%
%               \glsprintohnedeutsch%
%           }%
%       }%
%       %
%       \renewcommand*{\glsclearpage}{}%
%       %
%       \newlist{myglossarylist}{description}{10}%
%       \setlist[myglossarylist]{%
%           align=left,%
%       % 	itemindent=0em,%
%       % 	labelindent=0em,%
%       % 	listparindent=0em,%
%       }%
%       \setlist[myglossarylist,2]{%
%           align=left,%
%           leftmargin=2em,%
%           itemindent=-2em,%
%       }%
%       \newglossarystyle{list+url}
%       {% based on list style (adapt as required)
%         \setglossarystyle{list}%
%           \renewcommand{\glossentry}[2]{%
%           \item[\glsentryitem{##1}%
%                 \glstarget{##1}{\glossentryname{##1}}]
%              \glossentrydesc{##1}\glspostdescription\space##2%
%           \ifglshasfield{url}{##1}{\glspar
%            \glsletentryfield{\thisurl}{##1}{url}%
%            \expandafter\url\expandafter{\thisurl}}{}}%
%       }%
%       \newglossarystyle{list+Deutsch+Untertitel+alternativ+url}{%
%           \renewenvironment{theglossary}%
%               {\begin{myglossarylist}}{\end{myglossarylist}}%
%           \renewcommand*{\glossaryheader}{}%
%           \renewcommand*{\glsgroupheading}[1]{}%
%           \renewcommand*{\glossentry}[2]{%
%               \item[\glsentryitem{##1}%
%                     \glstarget{##1}{\glossentryname{##1}}]%
%       %
%               \ifglshasfield{untertitel}{##1}{\normalfont%
%                   \textbf{(}\glsentryuntertitel{##1}\textbf{)}.\space}{}%
%               \ifglshasfield{alternativ}{##1}{\normalfont%
%                   Auch genannt: \textbf{\glsentryalternativ{##1}}.\space}{}%
%               \ifglshasfield{deutsch}{##1}{Zu Deutsch: %
%                   \textbf{\glsentrydeutsch{##1}}.\space}{}%
%               \glossentrydesc{##1}\glspostdescription\space ##2%
%           \ifglshasfield{url}{##1}{\glspar
%               \url{\glsentryurl{##1}}}{}%
%           }%
%           \renewcommand*{\subglossentry}[3]{%
%               \begin{myglossarylist}%
%                   \item[\glssubentryitem{##2}%
%                   \glstarget{##2}{\strut\glossentryname{##2}%
%                   }]%
%       %
%                   \ifglshasfield{untertitel}{##2}{\normalfont%
%                       \textbf{(}\glsentryuntertitel{##2}\textbf{)}.\space}{}%
%                   \ifglshasfield{alternativ}{##2}{\normalfont%
%                       Auch genannt: \textbf{\glsentryalternativ{##2}}.\space}{}%
%                   \ifglshasfield{deutsch}{##2}{Zu Deutsch: %
%                       \textbf{\glsentrydeutsch{##2}}.\space}{}%
%                   \glossentrydesc{##2}\glspostdescription\space ##3.%
%               \end{myglossarylist}%
%           }%
%           \renewcommand*{\glsgroupskip}{\ifglsnogroupskip\else\indexspace\fi}%
%       }%
%       \setglossarystyle{list}%
%
% \setacronymstyle{long-short}
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							Glossaries fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%							Setups für enumitem
%					Lists - (itemize, enumerate, description)
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
% \setlist[1]{\labelindent=\parindent} % < Usually a good idea
%\setlist[description]{font=\sffamily\bfseries} % the Default
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							enumitem fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Setups für Hyperref/URL
%		Note: Package hyperref internally laods package url
%		(Like some other Packages do. For Example: biblatex)
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%\mathchardef\UrlBreakPenalty=100% I think default is 100
% Allow linebreaks in URLs after additional character to the defaults, but
% don't just \renew or \def it, because this would remove all characters
% predefined within \UrlBreaks in the package. This could mislead other users.
% E.g. can cause smaller dots.. So use the etoolbox with "append to"
%\appto\UrlBreaks{%
%	\do\*%
% 	\do\-% Is done with the url option "hyphens"
%	\do\~%
%	\do\"%
%	\do\a\do\b\do\c\do\d\do\e\do\f\do\g\do\h\do\i\do\j%
%	\do\k\do\l\do\m\do\n\do\o\do\p\do\q\do\r\do\s\do\t\do\u\do\v\do\w%
%	\do\x\do\y\do\z%
%}%
%	Note: Alread inside the \UrlBreaks by default are:
% 	\do\.%
% 	\do\=%
% 	\do\'%
% 	\do\&%
% 	\do\-% With the option hypens
% \expandafter\def\expandafter\UrlBreaks\expandafter{\UrlBreaks% save the current one
% 	\do\*%
% 	\do\-%
% 	\do\~%
% 	\do\'%
% 	\do\"%
% 	\do\-%
% 	\do\&%
% 	\do\=%
% }%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Hyperref/URL fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Redefinition of \texttt
%				to allow a proper hyphenation (Silbentrennung)
% other breakpoint symbols can be added, for example, below I also make [ a breakpoint:
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%\let\stdtexttt\texttt
% \newcommand{\newtexttt}[1]{%
%   \begingroup
%   \ttfamily
%   \begingroup\lccode`~=`/\lowercase{\endgroup\def~}{/\discretionary{}{}{}}%
%   \begingroup\lccode`~=`[\lowercase{\endgroup\def~}{[\discretionary{}{}{}}%
%   \begingroup\lccode`~=`.\lowercase{\endgroup\def~}{.\discretionary{}{}{}}%
%   \catcode`/=\active\catcode`[=\active\catcode`.=\active
%   \scantokens{#1\noexpand}%
%   \endgroup
% }
% Oh noes, better way: Look at the Schriftart Segment in the Header
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Redef fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Definitionen allgemeiner Farben
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%\definecolor{optionalargscolor}{RGB}{255,125,25}%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%							Farben fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%
%
%
%
% Initialisierungen wie Counter, Theorem, Variablen, Konstanten..
%
%\theoremstyle{break}
%\theoremheaderfont{\bfseries}
%\theorembodyfont{\normalfont}
%\theoremseparator{}
%\theorempreskip{0ex}
%\theorempostskip{0ex}
%\theoremindent0.5em
%
%
% 
% 
%
%

==> Feasibility Study on Virtual Process Controllers as Basis for Future Industrial Automation Systems (ICIT 2021, DL 30.11.2020)/supply/glossaries.tex <==
%________________________________________________________________________
%------------------------------------------------------------------------
%					Custom Key Definitions
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\%
\glsaddkey*{url}%Key Name
% {\glsentrytext{\glslabel}deutsch}%Default Value
{}%Default Value
{\glsentryurl}%Use analog \glsentrytext
{\Glsentryurl}%Use analog \Glsentrytext
{\glsurl}%Use analog \glstext
{\Glsurl}%Use analog \Glstext
{\GLSurl}%Use analog \GLStext%
%
\glsaddkey*{longpltwo}%Key Name
% {\glsentrytext{\glslabel}deutsch}%Default Value
{}%Default Value
{\glsentrylongpltwo}%Use analog \glsentrytext
{\Glsentrylongpltwo}%Use analog \Glsentrytext
{\glslongpltwo}%Use analog \glstext
{\Glslongpltwo}%Use analog \Glstext
{\GLSlongpltwo}%Use analog \GLStext%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%					Custom Key Definitions fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Glossar
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\newglossaryentry{}{%
	name={},%
	plural={},%
	description={},%
}%
%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Glossar fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Akronyme (Abkürzungen)
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
\newacronym{dmz}{DMZ}{demilitarized zone}
\newacronym{it}{IT}{information technology}
\newacronym{ot}{OT}{operational technology}
\newacronym{opcua}{OPC UA}{Open Platform Communications Unified Architecture}
\newacronym{tsn}{TSN}{time-sensitive networking}
\newacronym{scada}{SCADA}{supervisory control and data acquisition}
\newacronym{vpc}{VPC}{Virtual Process Controller}
\newacronym{plc}{PLC}{programmable logic controller}
\newacronym{udp}{UDP}{User Datagram Protocol}
\newacronym{pubsub}{Pub/Sub}{Publish/Subscribe}
\newacronym{vm}{VM}{virtual machine}
%\newacronym{IEEE}[IEEE]{Institute of Electrical and Electronics Engineers}
\newacronym{pc}{PC}{personal computer}
\newacronym{ptp}{PTP}{Precision Time Protocol}
\newacronym{ntp}{NTP}{Network Time Protocol}
\newacronym{splc}{Soft-PLC}{Software-PLC}
\newacronym{rte}{RTE}{Real-Time Ethernet}
\newacronym{osi}{OSI}{Open Systems Interconnection}
\newacronym{mac}{MAC}{Media Access Control}
\newacronym{e2e}{E2E}{end-to-end}
\newacronym{tcp}{TCP}{Transmission Control Protocol}
\newacronym{hmi}{HMI}{Human-Machine Interface}
\newacronym{kpi}{KPI}{Key Performance Indicator}
\newacronym{mes}{MES}{Manufacturing Execution System}
\newacronym{rami4.0}{RAMI 4.0}{Reference Architectural Model Industrie 4.0}
\newacronym{tacnet4.0}{TACNET 4.0}{Tactile Internet 4.0}
\newacronym{3gpp}{3GPP}{3rd Generation Partnership Project}
\newacronym{5gppp}{5GPPP}{5G Infrastructure Public Private Partnership}
\newacronym{itu}{ITU}{International Telecommunication Union}
\newacronym{ngnm}{NGNM}{Next Generation Mobile Networks}
\newacronym{agv}{AGV}{automated guided vehicle}
\newacronym{v2v}{V2V}{vehicle-to-vehicle}
\newacronym{v2x}{V2X}{vehicle-to-infrastructure}
\newacronym{d2x}{D2X}{device-to-x}
\newacronym{qos}{QoS}{quality of service}
\newacronym{noa}{NOA}{NAMUR Open Architecture}
\newacronym{dcs}{DCS}{distributed control system}
\newacronym{m2m}{M2M}{machine-to-machine}
\newacronym{sdn}{SDN}{software-defined networking}
\newacronym{erp}{ERP}{enterprise resource planning}
\newacronym{ip}{IP}{Internet Protocol}
\newacronym{lte}{LTE}{Long Term Evolution}
\newacronym{5g}{5G}{5th generation wireless communication system}
\newacronym{harq}{HARQ}{Hybrid Automatic Repeat Request}
\newacronym{rat}{RAT}{radio access technology}
\newacronym{mc}{MC}{Multi-Connectivity}
\newacronym{fbmc}{FBMC}{Filter Bank Multicarrier}
\newacronym{gfdm}{GFDM}{Generalized Frequency Division Multiplexing}
\newacronym{sla}{SLA}{service-level agreement}
\newacronym{5qi}{5QI}{5G QoS Indicator}
\newacronym{bmbf}{BMBF}{German Federal Ministry of Education and Research}
\newacronym{nrt}{NRT}{non real-time}
\newacronym{irt}{IRT}{isochronous real-time}
\newacronym{rt}{RT}{real-time}
\newacronym{ar}{AR}{augmented reality}
\newacronym{wlan}{WLAN}{wireless local area network}
\newacronym{cpu}{CPU}{central processing unit}
\newacronym{ram}{RAM}{random-access memory}
\newacronym{ue}{UE}{user equipment}
\newacronym{ran}{RAN}{radio access network}
\newacronym{bs}{BS}{base station}
\newacronym{cn}{CN}{core network}
\newacronym{epc}{EPC}{evolved packet core}
\newacronym{mec}{MEC}{mobile edge cloud}
\newacronym{rtt}{RTT}{round-trip time}
\newacronym{vpn}{VPN}{virtual private network}
\newacronym{vpf}{VPF}{Virtual Process Control Function}
\newacronym{vdi}{VDI}{Association of German Engineers}
\newacronym{ipc}{IPC}{industrial pc}
\newacronym{rtos}{RTOS}{real-time operating system}
\newacronym{vpcmo}{VPC M\&O}{VPC Management \& Orchestration}
\newacronym{i/o}{I/O}{input /output}
\newacronym{fbd}{FBD}{Function Block Diagram}
\newacronym{ldd}{LDD}{Ladder Logic Diagram}
\newacronym{sfc}{SFC}{Sequential Function Chart}
\newacronym{il}{IL}{Instruction List}
\newacronym{st}{ST}{Structured Text}
\newacronym{os}{OS}{operating system}
\newacronym{ir}{IR}{Inactive Resource}
\newacronym{msc}{MSC}{message sequence chart}
\newacronym{icps}{ICPS}{industrial cyber-physical system}
\newacronym{cps}{CPS}{cyber-physical systems}
\newacronym{mtd}{MTD}{Moving Target Defense}
\newacronym{iot}{IoT}{Internet of Things}
\newacronym{iiot}{IIoT}{industrial Internet of Things}
\newacronym{iiot2}{IIoT}{Industrial IoT}
\newacronym{k8s}{K8s}{Kubernetes}
\newacronym{rkt}{rkt}{CoreOS Rocket}
\newacronym{dcos}{DC/OS}{Distributed Cloud Operating System}
\newacronym{ml}{ML}{machine learning}
\newacronym{ai}{AI}{artificial intelligence}
\newacronym{ict}{ICT}{industrial communication technology}
\newacronym{kvm}{KVM}{kernel-based virtual machine}
\newacronym{ie}{IE}{Industrial Ethernet}
\newacronym{ias}{IAS}{industrial automation system}
\newacronym{cots}{COTS}{commercial off-the-shelf}
\newacronym{slat}{SLAT}{Second Level Address Translation}
\newacronym{gui}{GUI}{graphical user interface}
\newacronym{l2}{L2}{layer 2}
\newacronym{l3}{L3}{layer 3}
%\newacronym[plural=SDNs,%
	%firstplural=Software-Defined Networks (SDNs),%
	%longplural=Software-Defined Networks]%
	%{sdn}{SDN}{Software-Defined Network}%
%\glsunset{sdn}%
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Akronyme fertig
%------------------------------------------------------------------------
%________________________________________________________________________
%
%
%
%
%
%
%________________________________________________________________________
%------------------------------------------------------------------------
%						Dual Entrys
%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
% new makro, to easy create a DualEntry for Acronym references Glossary Entry
% -- Version 1:
% \newcommand*{\newdualentry}[5][]{%
% 	\newglossaryentry{gls-#2}{name={#4},text={#3\glsadd{#2}},%
% 		description={#5},#1%
% 	}%
% 	\newacronym{#2}{#3\glsadd{gls-#2}}{#4}%
% }%
% -- Version 2:
% (based on package xparse)

%\DeclareDocumentCommand{\newdualentry}{ O{} O{} m m m m }{%
%	\newglossaryentry{gls-#3}{name={#5\glsadd{#3}},%
%		text={#5},%
%		description={#6},#1}%
%	\newacronym[see={[Glossar:]{gls-#3}},#2]{#3}{#4\glsadd{gls-#3}}{#5}%
%}%

% Usage Syntax:
% \newdualentry[glossary options][acronym options]{label}{abbrv}{long}{description}
% and for the references:
% Refer to acronym with \gls{label} and the glossary with \gls{gls-label}
%________________________________________________________________________
%						Dual Entry Definitions
%VVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVVV

%\newdualentry%
%[]% Options für Glossary
%[]% Options für Acronym
%{QoS}% label
%{QoS}% abbreviation
%{Quality of Service}% long form
%{}% description

%/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\/\
%						Dual Entrys fertig
%-------------------------------------------------------------------------
%_________________________________________________________________________
%


==> organization/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Michael Gundall\IEEEauthorrefmark{1},\\%
    %Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%








% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/_templates/IEEE_authors-long.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1}, %
    Christoph Fischer\IEEEauthorrefmark{2}, %
    \\%
    FirstName1 Lastname1\IEEEauthorrefmark{3} and %
    FirstName2 Lastname2\IEEEauthorrefmark{4}%
}%
\IEEEauthorblockA{%
    \IEEEauthorrefmark{1}\IEEEauthorrefmark{2}German Research Center for Artificial Intelligence GmbH (DFKI)%
%     Trippstadter Str. 122\\%
%     67663 Kaiserslautern\\%
	\\%
    \IEEEauthorrefmark{3}Institute1, %
    Some Subtitle 1 %
%     Optional Address, Germany%
    \\%
	\IEEEauthorrefmark{4}Corporation2, %
    Some Subtitle2, %
    Some more Subt2 %
%     Optional Address
    \\%
    Email: %
        \{\IEEEauthorrefmark{1}dennis.krummacker, %
        \IEEEauthorrefmark{2}christoph.fischer\}@dfki.de, %
        \\%
        \IEEEauthorrefmark{3}Mail1@domain1.de, %
        \IEEEauthorrefmark{4}Mail2@domain2.com
}%
}%






% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/_templates/IEEE_authors.tex <==
% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{%
%
\IEEEauthorblockN{%
    Dennis Krummacker\IEEEauthorrefmark{1},\\%
    Christoph Fischer\IEEEauthorrefmark{2}%
}
\IEEEauthorblockA{%
    German Research Center for\\Artificial Intelligence GmbH, DFKI\\%
    Trippstadter Str. 122\\%
    67663 Kaiserslautern\\%
    Email: %{\tt
      \{%
        \IEEEauthorrefmark{1}dennis.krummacker,\\%
        \hspace*{1em}\IEEEauthorrefmark{2}christoph.fischer%
      \}@dfki.de
    %}%
}
%
\and%
%
\IEEEauthorblockN{%
    FirstName1 Lastname1\IEEEauthorrefmark{3},\\%
    FirstName2 Lastname2\IEEEauthorrefmark{4}
}%
\IEEEauthorblockA{%
	Chair of Something\\
    Faculty of Amazing Computer Science\\
    University\\
    Optional Address\\
    Email: \{\IEEEauthorrefmark{3}Mail1,\\ \hspace*{1em}\IEEEauthorrefmark{4}Mail2\}@domain.de
}%
}%
%
%









%\author{%
%           \IEEEauthorblockN{Michael Shell}
%           \IEEEauthorblockA{School of Electrical and\\Computer Engineering\\
%           Georgia Institute of Technology\\
%           Atlanta, Georgia 30332--0250\\
%           Email: http://www.michaelshell.org/contact.html}
%           \and
%           \IEEEauthorblockN{Homer Simpson}
%           \IEEEauthorblockA{Twentieth Century Fox\\
%           Springfield, USA\\
%           Email: homer@thesimpsons.com}
%           \and
%           \IEEEauthorblockN{James Kirk\\ and Montgomery Scott}
%           \IEEEauthorblockA{Starfleet Academy\\
%           San Francisco, California 96678--2391\\
%           Telephone: (800) 555--1212\\
%           Fax: (888) 555--1212}
%
%}%

% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}





==> organization/backing/IEEETemplateProvidedExamples.tex <==
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
% \begin{table}[!t]
% % increase table row spacing, adjust to taste
% \renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
% \caption{An Example of a Table}
% \label{table_example}
% \centering
% % Some packages, such as MDW tools, offer better commands for making tables
% % than the plain LaTeX2e tabular which is used here.
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{table}

==> organization/backing/thebibliography.tex <==
% can use a bibliography generated by BibTeX as a .bbl file
% BibTeX documentation can be easily obtained at:
% http://mirror.ctan.org/biblio/bibtex/contrib/doc/
% The IEEEtran BibTeX style support page is at:
% http://www.michaelshell.org/tex/ieeetran/bibtex/
%\bibliographystyle{IEEEtran}
% argument is your BibTeX string definitions and bibliography database(s)
%\bibliography{IEEEabrv,../bib/paper}
%
% <OR> manually copy in the resultant .bbl file
% set second argument of \begin to the number of references
% (used to reserve space for the reference number labels box)
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.
  
\bibitem{IEC61158}
, \emph{IEC 61158},

\bibitem{61158-trafficclass}
E DIN EN 61158-1:2017-09 11.4.2

\bibitem{61158-endpoint}
E DIN EN 61158-1:2017-09 9.3.3.3.1

\bibitem{62439-endnode}
DIN EN 62439-1:2010-09 3.1.13

\end{thebibliography}
